An Overview of Depth Cameras and Range Scanners Based on Time-of-Flight Technologies

Time-of-flight (TOF) cameras are sensors that can measure the depths of scene-points, by illuminating the scene with a controlled laser or LED source, and then analyzing the reflected light. In this paper, we will first describe the underlying measurement principles of time-of-flight cameras, including: (i) pulsed-light cameras, which measure directly the time taken for a light pulse to travel from the device to the object and back again, and (ii) continuous-wave modulated-light cameras, which measure the phase difference between the emitted and received signals, and hence obtain the travel time indirectly. We review the main existing designs, including prototypes as well as commercially available devices. We also review the relevant camera calibration principles, and how they are applied to TOF devices. Finally, we discuss the benefits and challenges of combined TOF and color camera systems.

==> cover_letter.tex <==
\begin{coverletter}{An Overview of Range Scanners and Depth Cameras\\ Based on Time-of-Flight Technologies}{MVAP-D-15-00350}



\begin{answereditor}
{Reviewers have now commented on your paper. You will see that they are advising that you revise your manuscript. If you are prepared to undertake the work required, I would be pleased to reconsider my decision.  
}
{We thank the reviewers for their useful comments. When we revised the submission we tried to take into account all their comments. The changes can be easily tracked by clicking on the corresponding links in the cover letter, for example \refcm{tof-calib}. The main revisions are the followings:
\begin{itemize}
\item We clarified some technical specifications of the Kinect~v2 camera based on \citep{bamji20150} which is now cited, \refcm{kinect-v2}.
\item All the reviewed cameras (18 different models from 9 manufacturers) appear in three different tables.
\item We revised our discussion on various methods for depth calibration, \refcm{depth-error}, and depth error detection, \refcm{multi-path}.
\item We discuss in more detail the advantages and disadvantages of \tof{} technologies and practical uses of these cameras, \refcm{tof-calib}, \refcm{lidar}, and \refcm{kinect-lim}.
\item As suggested by the reviewers we added and commented the following references:
\citep{bamji20150}, \citep{fursattel2015comparative}, \citep{son2016automatic}, \citep{kuznetsova2014calibration}, \citep{ferstllearning}, \citep{freedman2014sra}.
\end{itemize}
}
\end{answereditor}


\begin{answerreviewer}

\qa
{ The paper presents a description of some of the current technologies to obtain depth images, specifically range scanners and Time-of-Flight (ToF) cameras. The title and the abstract correspond to the contents of the paper: an overview. The paper in its current form is informative enough, but of low interest to the community. The paper could be of more interest if some criticism about the benefits/inconveniences of the different technologies, accuracy of the different alternatives, and calibration hints is added.
}
{All the range scanners and depth cameras overviewed in this paper are based on two time-of-flight principles (pulsed light and modulated light). We changed the order of ``range scanners" and ``depth cameras" in the title in order to remove this apparent confusion. We don't agree with the reviewer that the content of the paper is of low interest to the ``community". We are not aware of an article that gathers in a concise and precise way the physical and electronics principles of both pulsed-light and modulated-light TOF cameras and scanners. In particular, the description of the principles of these cameras can be found in many articles and textbooks, but a concise overview is not currently available.\\

We added some more criticisms concerning the various TOF technologies (please consult \refcm{tof-calib}, \refcm{lidar}, and \refcm{kinect-lim}), but this is not the primary scope of this paper. We cite some recent references that address the issues of depth errors and depth accuracy. Following the advice of the reviewer we revised Section 6 (Calibration).}


\qa
{The description of the electronic principles (Sec. 2) is interesting but not sure if is of the interest of MVAP readers. My main concern is that only a description but no conclusions is presented: which are the real effects on the obtained image (pros/cons) of using this technology; comparison versus some alternative (if any); errors and side effects produced when used (like interferences between pixelsÉ).}
{We don't agree. The electronic principles allow the reader to understand the technology and its fundamental limitations. Concerning the pulsed-light systems, we discuss both the limitation in terms of pixel size and in terms of range accuracy (Section 2). To the best of our knowledge, the demodulation principles that are used by continuous-wave cameras (Section 4.1) cannot be found in any of the articles describing this type of cameras -- this was overlooked. }

 \qa
{The calibration section does not review the relevant procedures. One page is devoted to the wellÑknown calibration procedures shared with color cameras (Secs. 6.1, 6.2, 6.3), while less than one column (Sec. 6.4) is devoted to the specific calibration of the depth. The paper would be of more interest if the specificity of the ToF cameras are revealed (low resolution, depth calibration).  A discussion of the efforts of the manufacturers to provide already-calibrated cameras would provide valuable information to readers, and enhance the possibility of obtain more cites. I appreciate the practical considerations (Sec. 6.5) and encourage authors to expand this section.}
{We believe that it is important to summarize the basic color-camera calibration model and method because they are shared by all the TOF calibration methods. Concerning depth calibration, we added several references to recent articles that estimate depth errors, as well as a recent review article that compares several (eight) TOF cameras via an error analysis, \refcm{depth-error}. Concerning the efforts of manufacturers, we now introduce a description of the multiple-frequency design of the Kinect~v2 that improves depth accuracy, \refcm{kinect-v2}. As suggested by the reviewer, we expanded Section 6.5 with a discussion on multiple-path errors, \refcm{multi-path}, and with citations to several recent papers, including a recent comparative study.}

\qa
{The description of the cameras does not include some valuable information. The most important one,  which is the quality of the obtained images? All cameras produce equally precise depth readings? All the pixels of the image generate equally precise depth readings? 

It could be nice if the reader can find the answer to this question: Which camera/technology I should choose for my application? Currently, the answer is only partially answered based on its availability on the market.
}
{Choosing a \tof{} camera for a specific application is a difficult question to answer. This choice depends on many factors, such as the product availability, budget, indoor or outdoor application, range, scene complexity, ambient light, ease of calibration, etc. The approach taken by the authors in the current submission is to explain the fundamental principles of \tof{} technologies, whether pulsed-light or continuous-wave, together with their intrinsic advantages and disadvantages, and this independently of the targeted application. We believe that Section 8 gathers some general \tof{} camera and scanner features to be taken into account for choosing a particular \tof{} technology.}

\qa
{Some minor comments:

pp.6-l50: A reference is required to the NASA experiments.

pp.7-l33: Figure 7 depicts the image formation process, but not its "architecture".}
{We added a reference to the NASA experiments, \citep{amzajerdian2011lidar}. We revised the caption of Figure 7.}

\end{answerreviewer}


\begin{answerreviewer}
\qa
{The authors present an overview paper for Time-of-Flight based range scanners. The overview includes pulsed and continuous wave time-of-flight as well as LIDAR. Furthermore some calibration theory is presented.

In general the paper just describes / summarizes information which has been available for a long time. }
{It is true that the paper summarizes information available elsewhere. This is exactly the goal of this overview paper. We are not aware of an article that summarizes all the time-of-flight technologies that are available today. We believe that such an overview is quite useful for computer vision and image processing practitioners, by providing a broad view of the basic principles of time of flight imaging.}

\qa
{2.1. Avalanche diodes.
This section might be hard to understand for readers with a computer vision/algorithm background}
{This section is probably one of the most important ones because it summarizes the basic principle of avalanche diode. We assume that the MVAP readers know what is a ``diode" and this is the only background in applied physics and electronics that is needed to understand this section. Moreover, this section allows the reader to understand the basic limitations of sensors based on SPADs in terms of spatial resolution.}

 \qa
{5.2. The Kinect v2 RGB-D Camera.
The presented information about the Kinect v2 is not correct. It is stated, that the Kinect is able to generate depth data up to 4.5m. Correct is that the Kinect is able to acquire depth data up to 8m and body tracking is only provided for up to 4.5m. Also the conclusion about the modulation frequency does not make sense. Information about the sensor can be found here: http://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=6964815}
{Thank you for providing a link to a recent scientific publication that describes the Kinect v2 camera. We corrected the information about the camera specifications based on \citep{bamji20150}. The updated figures that we provide in our submission correspond to those to be found in Table~I of \citep{bamji20150}, \refcm{kinect-v2}.}

\qa
{5.3. Other CW ToF Cameras.
Clarify that there exist more cameras than the ones listed in the draft.}
{This is now clarified twice: \refcm{commercial} and \refcm{commercial-cw}.}

\qa
{6.4. Depth Distortion
There exist a couple of different error sources which deteriorate the ToF measurements. With the current document the reader may get the impression that wiggling is the dominant error. It should be emphasized that there exist additional errors, including amplitude-related errors, internal scattering, temperature-related errors and multi-path effects. Descriptions of these errors are given in "Foix et. al, 2011", which has already been cited.
A recent evaluation of ToF-cameras, which demonstrates the occurrence of these errors, can be found in "FŸrsattel et. al, 2015, A Comparative Error Analysis of Current Time-of-Flight Sensors".}
{One has to make a clear distinction between the scientific and technological foundations of TOF cameras and scanners, on one side, and the actual depth measurements obtained in practice, on the other side. We now cite the paper \citep{fursattel2015comparative} which offers a comparative error analysis of some commercially available TOF sensors. We note that \citep{fursattel2015comparative} treats the cameras as ``black boxes" and the comparison covers CW TOF cameras only. Hence, the current submission and \citep{fursattel2015comparative} are complementary.}

\qa
{For some of the available systems resolution, accuracy and related information is presented in corresponding tables. However this information is not available for all presented systems. The authors should include this information or at least tell why it is not available.
}
{In the revised submission we incorporated three tables: TOF scanners based on pulsed light (Table I), 3D Flash cameras based on pulsed light (Table II) and continuous-wave cameras based on modulated light (Table III).}

\qa
{For completeness the authors should also consider recent Panasonic chips which are commercially available in Basler cameras and Fotonic cameras\\ (see https://www.baslerweb.com/media/documents/BAS1409\_ToF\_EN\_web.pdf)}
{We incorporated information about the Basler camera which uses pulsed light (Table II). We could not find detailed information about the Panasonic chips. The Fotonic cameras were already included in our overview. }

\qa
{There also exist more recent correction methods for ToF sensors, which apply machine learning techniques to better model the errors which occur with ToF sensors. Examples include:
"Son et. al, 2016, Automatic Learning to Remove Multipath Distortions in Time-of-Flight Range Images for a Robotic Arm Setup" and
"Ferstl et. al, 2015, Learning Depth Calibration of Time-of-Flight Cameras"

In contrast to the previously mentioned machine-learning approaches, one can also use kernel-regression approaches to cope with the measurement errors, like shown in "Kuznetsova, 2013, On calibration of a low-cost time-of-flight camera".}
{We included all these references and discussed them. In our discussion we make a clear distinction between the use of machine learning techniques (mainly regression methods) to correct depth errors, \refcm{depth-error}, and multiple path detection and correction, \refcm{multi-path}. }


\end{answerreviewer}

\end{coverletter}

